MQT-TZ: Secure MQTT Broker for Biomedical Signal Processing on the Edge

Physical health records belong to healthcare providers, but the information contained within belongs to each patient. In an increasing manner, more health-related data is being acquired by wearables and other IoT devices following the ever-increasing trend of the "Quantified Self". Even though data protection regulations (e.g., GDPR) encourage the usage of privacy-preserving processing techniques, most of the current IoT infrastructure was not originally conceived for such purposes. One of the most used communication protocols, MQTT, is a lightweight publish-subscribe protocol commonly used in the Edge and IoT applications. In MQTT, the broker must process data on clear text, hence exposing a large attack surface for a malicious agent to steal/tamper with this health-related data. In this paper, we introduce MQT-TZ, a secure MQTT broker leveraging Arm TrustZone, a popular Trusted Execution Environment (TEE). We define a mutual TLS-based handshake and a two-layer encryption for end-to-end security using the TEE as a trusted proxy. We provide quantitative evaluation of our open-source PoC on streaming ECGs in real time and highlight the trade-offs.

==> figs/handshake-algorithm.tex <==
\begin{algorithm}[t!]
    \floatname{Protocol}{Two-Step Handshake}
    \renewcommand{\thealgorithm}{}
    \caption{Steps that Mallory follows to hjobtain key K}
    \label{protocol1}
    \begin{algorithmic}[1]
    \STATE $M$ : Eavesdrops the protocol 1 above and gets $X$ from step 1 and initiates the same protocol with $B$, by substituting $X$ for $K$ above.
    \STATE $M\rightarrow{B}$ : $P = E_{B}(S_{M}(X)) = E_{B}(S_{M}(E_{B}(S_{A}(K))))$
    \STATE $B$ : $V_{M}(D_{B}(P)) = V_{A}(D_{B}(E_{B}(S_{A}(X)))) = X$
    \STATE $B\rightarrow{M}$ : $Q = E_{M}(S_{B}(X)) = E_{M}(S_{B}(E_{B}(S_{A}(K))))$\\
    Since the same key pair is used for both encryption and signing, $S_{B}(E_{B}(message)) = message$\\
    Therefore, $Q = E_{M}(S_{A}(K))$
    \STATE $M$ : $D_{M}(Q) = S_{A}(K)$
    \STATE $M$ : Since the same key pair is used for both encryption and signing, $E_{A}(S_{A}(K)) = K$. Mallory can obtain the key $K$ in this way and decrypt all the subsequent messages encrypted with key $K$.
    \end{algorithmic}
\end{algorithm} 


==> figs/tls-handshake.tex <==
\begin{sequencediagram}
    \newthread{cli}{Client}
    \newinst[1]{ca}{CA (Let's Encrypt)}
    \tikzstyle{inststyle}+=[top color=gray!30, bottom color=gray!30]
    \newinst[1]{b-ns}{Broker (NS)}
    \tikzstyle{inststyle}+=[top color=gray!60, bottom color=gray!60]
    \newinst{b-s}{Broker (S)}
    \begin{sdblock}{TLS-HS}{TLS Handshake - Broker (Server) Authentication Only}
        \begin{call}{cli}{\small{\texttt{Hello(cliTLSProps)}}}{b-ns}{\small{\texttt{Hello(chosenTLSProps, brkCert)}}}
        \end{call}
        \begin{call}{cli}{\small{\texttt{Trust(brkCert)}}}{ca}{\small{\texttt{Y/N}}}
        \end{call}
    \end{sdblock}
    %\begin{sdblock}{\tiny{\texttt{Key Exchange}}}{\tiny{\texttt{Key Exchange}}}
    \begin{sdblock}{Cli-Auth}{Client Authentication w/ TZ-Specific Key over MQTT}
        \begin{call}{cli}{\small{\texttt{Enc(cliSK,brkPK)}}}{b-ns}{\small{\texttt{Send(encData)}}}
            \begin{call}{b-ns}{\tiny{\texttt{Send(encData)}}}{b-s}{\tiny{\texttt{Enc(OK, cliSKey)}}}
                \begin{call}{b-s}{\tiny{\texttt{Dec(encData,brkpK)}}}{b-s}{}
                \end{call}
                \begin{call}{b-s}{\tiny{\texttt{SecureStore(cliSK)}}}{b-s}{}
                \end{call}
            \end{call}
        \end{call}
    \end{sdblock}
\end{sequencediagram}

